Producibility in hierarchical self-assembly

Three results are shown on producibility in the hierarchical model of tile self-assembly. It is shown that a simple greedy polynomial-time strategy decides whether an assembly A is producible. The algorithm can be optimized to use O(|A| log^2 |A|) time. Cannon, Demaine, Demaine, Eisenstat, Patitz, Schweller, Summers, and Winslow showed that the problem of deciding if an assembly A is the unique producible terminal assembly of a tile system T can be solved in O(|A|^2 |T| + |A| |T|^2) time for the special case of noncooperative "temperature 1" systems. It is shown that this can be improved to O(|A| |T| log |T|) time. Finally, it is shown that if two assemblies are producible, and if they can be overlapped consistently -- i.e., if the positions that they share have the same tile type in each assembly -- then their union is also producible.

==> intro-dolemite.tex <==
\vspace{-1.1cm}
\section{Introduction}
\label{sec-intro}

\subsection{Background of the field}
Winfree's abstract Tile Assembly Model (aTAM)~\cite{Winfree98simulationsof} is a model of crystal growth through cooperative binding of square-like monomers called \emph{tiles}, implemented experimentally (for the current time) by DNA~\cite{WinLiuWenSee98, BarSchRotWin09}.
In particular, it models the potentially algorithmic capabilities of tiles that can be designed to bind if and only if the total strength of attachment (summed over all binding sites, called \emph{glues} on the tile) is at least a parameter $\tau$, sometimes called the \emph{temperature}.
In particular, when the glue strengths are integers and $\tau=2$, this implies that two strength 1 glues must cooperate to bind the tile to a growing assembly.
Two assumptions are key: 1) growth starts from a single specially designated \emph{seed} tile type, and 2) only individual tiles bind to an assembly, never larger assemblies consisting of more than one tile type.
We will refer to this model as the \emph{seeded aTAM}.
While violations of these properties are often viewed as errors in implementation of the seeded aTAM~\cite{SchWin07, SchWin09}, relaxing the assumptions results in a different model with its own programmable abilities.
In the \emph{hierarchical} (a.k.a. \emph{multiple tile}~\cite{AGKS05}, \emph{polyomino}~\cite{Winfree06, Luhrs10}, \emph{two-handed}~\cite{TwoHandsBetterThanOne, DotPatReiSchSum10, TwoHandedNotIntrinsicallyUniversalconf}) \emph{aTAM}, there is no seed tile, and an assembly is considered producible so long as two producible assemblies are able to attach to each other with strength at least $\tau$, with all individual tiles being considered as ``base case'' producible assemblies.
In either model, an assembly is considered \emph{terminal} if nothing can attach to it; viewing self-assembly as a computation, terminal assembly(ies) are often interpreted to be the output.
See~\cite{DotCACM} for an introduction to recent work in these models.

The hierarchical aTAM has attracted considerable recent attention.
%
It is $\coNP$-complete to decide whether an assembly is the unique terminal assembly produced by a hierarchical tile system~\cite{TwoHandsBetterThanOne}.
%
There are infinite shapes that can be assembled in the hierarchical aTAM but not the seeded aTAM, and vice versa, and there are finite shapes requiring strictly more tile types to assemble in the seeded aTAM than the hierarchical aTAM, and vice versa~\cite{TwoHandsBetterThanOne}.
%
Despite this incomparability between the models for exact assembly of shapes, with a small blowup in scale, any seeded tile system can be simulated by a hierarchical tile system~\cite{TwoHandsBetterThanOne}, improving upon an earlier scheme that worked for restricted classes of seeded tile systems~\cite{Luhrs10}.
%
However, the hierarchical aTAM is not able to simulate itself from a single set of tile types, i.e., it is not \emph{intrinsically universal}~\cite{TwoHandedNotIntrinsicallyUniversalconf}, unlike the seeded aTAM~\cite{TAMIU}.
%
It is possible to assemble an $n \times n$ square in a hierarchical tile system with $O(\log n)$ tile types that exhibits a very strong form of fault-tolerance in the face of spurious growth via strength 1 bonds~\cite{DotPatReiSchSum10}.
%
The parallelism of the hierarchical aTAM suggests the possibility that it can assemble shapes faster than the seeded aTAM, but it cannot for a wide class of tile systems~\cite{CheDot12}.

Interesting variants of the hierarchical aTAM introduce other assumptions to the model.
The \emph{multiple tile} model retains a seed tile and places a bound on the size of assemblies attaching to it~\cite{AGKS05}.
%
Under this model, it is possible to modify a seeded tile system to be \emph{self-healing}, that is, it correctly regrows when parts of itself are removed, even if the attaching assemblies that refill the removed gaps are grown without the seed~\cite{Winfree06}.
%
The model of \emph{staged assembly} allows multiple test tubes to undergo independent growth, with excess incomplete assemblies washed away (e.g. purified based on size) and then mixed, with assemblies from each tube combining via hierarchical attachment~\cite{DDFIRSS07, DemEisIshWinOneDimStagedjournal}.
%
The \emph{RNase enzyme} model~\cite{RNaseSODA2010, DemPatSchSum2010RNase, PatSumIdentifyingJournal} assumes some tile types to be made of RNA, which can be digested by an enzyme called RNase, leaving only the DNA tiles remaining, and possibly disconnecting what was previously a single RNA/DNA assembly into multiple DNA assemblies that can combine via hierarchical attachment.
%
Introducing negative glue strengths into the hierarchical aTAM allows for ``fuel-efficient'' computation~\cite{SchSheSODAFuel}.




\subsection{Contributions of this paper}
We show three results related to producibility in the hierarchical aTAM.
\begin{enumerate}
  \item
  In the seeded aTAM, there is an obvious linear-time algorithm to test whether assembly $\alpha$ is producible by a tile system: starting from the seed, try to attach tiles until $\alpha$ is complete or no more attachments are possible.
  We show that in the hierarchical aTAM, a similar greedy strategy correctly identifies whether a given assembly is producible, though it is more involved to prove that it is correct.
  The idea is to start with all tiles in place as they appear in $\alpha$, but with no bonds, and then to greedily bind attachable assemblies until $\alpha$ is assembled.
  The algorithm can be optimized to use $O(n \log^2 n)$ time.
  It is not obvious that this works, since it is conceivable that assemblies must attach in a certain order for $\alpha$ to form, but the greedy strategy may pick another order and hit a dead-end in which no assemblies can attach.
  This is shown in Section~\ref{sec-algorithm}.

  \item
  We show that there is a faster algorithm for the temperature 1 Unique Production Verification (UPV) problem studied by Cannon, Demaine, Demaine, Eisenstat, Patitz, Schweller, Summers, and Winslow~\cite{TwoHandsBetterThanOne}, which is the problem of determining whether assembly $\alpha$ is the unique producible terminal assembly of tile system $\calT$, where $\calT$ has temperature 1, meaning that all positive glue strength are sufficiently strong to attach any two assemblies.
  They give an algorithm that runs in $O(n^2)$ time.
  We show how to improve this running time.
  Cannon et al.~proved their result by using an $O(n^2)$ time algorithm for UPV that works in the seeded aTAM~\cite{ACGHKMR02}, and then reduced the hierarchical temperature-1 UPV problem to instances of the seeded UPV problem.
  We improve this result by showing that a faster $O(n \log n)$ time algorithm for the seeded UPV problem exists for the special case of temperature 1, implying that the algorithm of Cannon et al.~for the hierarchical model can thus be made to run in $O(n \log n)$ time.
  This is shown in Section~\ref{sec-upv-t1}.
  %We also show a direct (and simpler) $O(n)$ time algorithm for the hierarchical temperature-1 UPV problem.
  %We include the former algorithm because the seeded result may be of independent interest.
  %In particular, the connection between mismatches and biconnected components of the binding graph may have implications for an open question~\cite{DotPatSum11} regarding the computational power of the seeded temperature 1 aTAM.

  \item
  We show that if two assemblies $\alpha$ and $\beta$ are producible in the hierarchical model, and if they can be overlapped consistently (i.e., if the positions that they share have the same tile type in each assembly), then their union $\alpha \cup \beta$ is producible.
  This is trivially true in the seeded model, but it requires much more care to prove in the hierarchical model.
  It is conceivable \emph{a priori} that although $\beta$ is producible, $\beta$ must assemble $\alpha \cap \beta$ in some order that is inconsistent with how $\alpha$ assembles $\alpha \cap \beta$.
  This is shown in Section~\ref{sec-union}.
\end{enumerate}


